Why Did My Query Slow Down?

Many enterprise environments have databases running on network-attached server-storage infrastructure (referred to as Storage Area Networks or SANs). Both the database and the SAN are complex systems that need their own separate administrative teams. This paper puts forth the vision of an innovative management framework to simplify administrative tasks that require an in-depth understanding of both the database and the SAN. As a concrete instance, we consider the task of diagnosing the slowdown in performance of a database query that is executed multiple times (e.g., in a periodic report-generation setting). This task is very challenging because the space of possible causes includes problems specific to the database, problems specific to the SAN, and problems that arise due to interactions between the two systems. In addition, the monitoring data available from these systems can be noisy. We describe the design of DIADS which is an integrated diagnosis tool for database and SAN administrators. DIADS generates and uses a powerful abstraction called Annotated Plan Graphs (APGs) that ties together the execution path of queries in the database and the SAN. Using an innovative workflow that combines domain-specific knowledge with machine-learning techniques, DIADS was applied successfully to diagnose query slowdowns caused by complex combinations of events across a PostgreSQL database and a production SAN.

==> demo.tex <==


%\newpage

\section{Demonstration Proposal}
\label{sec:demo}

\begin{figure}[!t]
	\centering
	\includegraphics[clip=true,width=1\linewidth, height = 1.5in, viewport= 0 50 410 190]{Figures/demo_setup.eps}
	\caption{\dbtool{} demonstration setup}
	\label{fig:demo}
	\vspace{-5mm}
\end{figure}



%1 intro to the demo injecting faults and how diads work
%2 prototype system
%3 explain the experiments

In the demonstration  session, we will present \dbtool{} in action on both
live faults injected in a realistic DB/SAN environment, as well as on offline diagnosis;
tracking the reasoning process of the diagnosis workflow
by drilling down to the intermediate results like anomaly, confidence, and impact scores.
 Our demonstration setup is depicted in Figure \ref{fig:demo}. This setup consists of:

\squishlist

\item Data-warehousing queries from the
TPC-H benchmark running on a PostgreSQL database server 
configured to access data on an enterprise-class IBM storage controller.

\item The IBM TotalStorage Productivity Center (TPC) running on a
separate machine recording configuration details, statistics, and events
from the SAN as well as from PostgreSQL (which was instrumented to
report the data to the management tool). Figure~\ref{metrics-table}
shows the key performance metrics collected from the database and SAN.
The monitoring data is stored as time-series data in a DB2 database. 

\item \dbtool{}'s web-based front-end  running on a separate server. 
This front-end supports APG-oriented display and browsing of data collected 
in the DB2 database.  Recall that  APGs are views on the monitoring data that combine what DBAs
see---e.g., data on query plans---with what SAN administrators
see---data from the numerous SAN components and their
interconnections. APG-oriented visualization was implemented due to  comments from administrators 
that  to diagnose a reasonable fraction of problems all they need to see is the APG diagram. 
 
\item \dbtool{}'s diagnosis workflow which is invoked on demand. 
Each module in the workflow is implemented using 
a combination of Matlab scripts (for KDE) and Java. \dbtool{} uses 
a symptoms database that was developed in-house to handle query slowdowns.

\item A fault injector that can inject a variety of faults at the database 
and SAN levels, including SAN misconfiguration, server, disk, or volume contention,
RAID rebuilds, changes in data properties, and table-locking problems. 

\squishend 

\noindent \dbtool{} will be demonstrated through the scenarios  listed in Table \ref{table:exper}. 
For  the first scenario, we will show live fault injection, 
namely, a SAN misconfiguration that causes an external workload to use $V_1$, causing
contention. Because the demonstration period is short (10 minutes), the other scenarios will be
demonstrated without live fault injection. 
Note that \dbtool{} works off of data that is stored in the DB2 database outside of the system
being monitored. This property 
allows \dbtool{} to run and analyze query slowdowns offline, provided the 
required APG data from satisfactory and unsatisfactory runs 
has already been captured in the DB2 database. 

Diagnosis in each scenario starts with the administrator identifying 
a query that experienced a slowdown, as well as satisfactory and unsatisfactory 
runs of the query. The diagnosis workflow is then invoked. 
By default, the workflow is run in a {\em batch} mode where 
all modules are executed one after the other, 
and only the final results are displayed to the administrator. However, 
\dbtool{} supports an 
 {\em interactive} mode where results are displayed after each module completes,  
and the administrator can edit these results before they are fed to the 
next module. In this mode, the administrator  can also re-execute or 
bypass modules, as well as stop the execution if
the desired result is obtained quickly. Our demonstration will 
use the step-by-step interactive mode to give the audience 
maximum insight into how \dbtool{} works. 

The following features of \dbtool{} will be brought out as we work our way through the 
five scenarios in Table \ref{table:exper}:

\squishlist

\item {\em Dealing with event propagation:}
In Scenario \#3 in Table \ref{table:exper}, we cause a query slowdown by changing the 
properties of the data, causing extra I/O on Volume $V_2$.   
The change is done by an update statement that 
modifies the value of an attribute in some records of the {\em part} table.
The overall size of all tables, including {\em part}, are unchanged.
There are no external causes of contention on the volumes. In this scenario,
Module CR correctly identifies all the operators whose record-counts
show a correlation with plan performance, causing Module SD to list 
changes in data properties as a high-confidence cause. Module IA  
gives the final confirmation that 
the change in data properties is the root cause, and rules out
the presence of high-impact external causes of volume contention.

\item {\em Dealing with multiple concurrent problems:}
Scenarios \#2 and \#4 both have multiple concurrent problems occurring in the system. 
The difference between them is that in Scenario \#2 only one of the problems impacts the 
query performance, while in Scenario \#4 both problems 
impact query performance (albeit to different levels). \dbtool{} successfully
diagnoses the root cause(s) in both scenarios. We will contrast how \dbtool{} works 
in these two scenarios to showcase the importance of Modules DA and IA. 

\item {\em Dealing with noisy monitoring data:} 
Scenario \#5 has one real problem happening in the system. In addition, 
high levels of noise in the monitoring data cause symptoms corresponding
to a different problem to arise by chance. We will show how Module IA enables
\dbtool{} to generate the correct diagnosis result even in this challenging 
scenario. 


\squishend


